Region-based Content Enhancement for Efficient Video Analytics at the Edge

Video analytics is widespread in various applications serving our society. Recent advances of content enhancement in video analytics offer significant benefits for the bandwidth saving and accuracy improvement. However, existing content-enhanced video analytics systems are excessively computationally expensive and provide extremely low throughput. In this paper, we present region-based content enhancement, that enhances only the important regions in videos, to improve analytical accuracy. Our system, RegenHance, enables high-accuracy and high-throughput video analytics at the edge by 1) a macroblock-based region importance predictor that identifies the important regions fast and precisely, 2) a region-aware enhancer that stitches sparsely distributed regions into dense tensors and enhances them efficiently, and 3) a profile-based execution planer that allocates appropriate resources for enhancement and analytics components. We prototype RegenHance on five heterogeneous edge devices. Experiments on two analytical tasks reveal that region-based enhancement improves the overall accuracy of 10-19% and achieves 2-3x throughput compared to the state-of-the-art frame-based enhancement methods.

==> Highlight.tex <==
\section{Highlight}

% \textbf{Background:} Efficient Video analytics (at scale) on (Edge)
% \begin{enumerate}
%     \item 
%     \item 
% \end{enumerate}

% \textbf{Motivation:} \ding{172} Entire-frame SR is unnecessary. \ding{173} Redundancy in the temporal dimension.
% \begin{enumerate}
%     \item Intra-frame latency saving
%                 \begin{figure}[h]
%                 \centering
%                 \includegraphics[height=1.6in]{figs/cdf_2.pdf}
%                 \caption{Latency saving opportunities from spatial}
%                 \label{fig:spatiallatencysave}
%                 \end{figure}
%     \item Inter-frame latency saving under bounded accuracy drop by (Mask/Infer) results reuse. \wnote{TODO: FIGURE x-axis: frame index; y-axis: accuracy. EXPERIMENT: Object detection \& Semantic Segmentation}
%     \item Cross-stream coordination. To 1C+1G, we only need to reorder the queue of Mask+SR+detect+MV. To 1C+2/4G, instance-awareness (place each DNN per GPU) or stream-awareness (load streams on each GPU equally) are always inefficient. 
%     \item \ynote{In dense scenes, distant and small objects only occupy a few pixels. Need to be SRed.}
% \end{enumerate}

% \textbf{Goal:} Speed up E2E latency/throughput (with negligible accuracy drop).\wnote{Efficiency yet accurate}

% \textbf{Challenges:}
% We bypass the method of extracting features along both spatial and temporal dimensions [MGsampler CVPR21] by 3D conv, LSTM, or transformers as they are too heavy in real-time video analytics. Even though some works accelerate it by decomposing 3D convolution into 2D conv and 1D temporal conv [37,29]or integrating 2D conv into 3D [53], it is still computation hungry.
% \begin{enumerate}
    % \item How to distinguish important regions for CV accuracy in one frame? Previous heuristic methods are not robust. \wnote{TODO: experiment with on-board camera dataset.}
    % \item How to leverage the temporal redundancy?
    % % \item \sout{How to schedule the MASK/SR/Infer/Reuse jobs on CPU and GPU to make the best of the difference between display order and decoding order?}
%                     \begin{figure}[h]
%                     \centering
%                     %\setlength{\abovecaptionskip}{1.2pt}
%                     %\setlength{\belowcaptionskip}{0pt}
%                     \includegraphics[height=1.5in]{figs/Decodeorder.jpeg}
%                     \caption{Display \vs Decode order}
%                     \label{fig:StreamingCompare}
%                     \end{figure}
% \end{enumerate}

\textbf{Approaches:}
\begin{enumerate}
    % \item MB-level SR selection.
    % \begin{itemize}
    %     \item The reason on MB level.
    %     \item Metric to measure the importance of MB for accuracy. Mask* = $\sum_{i\in MB}\left|\left|\frac{ \partial Acc(D(F), D(SR(F))) }{ \partial IN(F) }\Big|_i\right|\right|_1 \cdot ||(SR(F)_i-F_i)||_1$
    %     \item DNN selection. Training setup. \wnote{TODO: PICTURE: 9 DNNs' performance}.
    % \end{itemize}
    \item MASK reuse. \wnote{Find an existing feature 
    % \sout{in the bitstream} 
    to measure the change of MASK* with correlation ratio >0.9.}  
    \begin{itemize}
        \item  We can use $l_1$-norm to transfer the difference into \underline{distribution}, then \underline{uniformly choose} the frames according to the distribution subject to the Latency Budget $B$. \jnote{However, with this method, we should \underline{update} the distribution of remaining frames based on the influence of the frame selected.}\wnote{We may use some \underline{Conditional Distribution} to update.} 
        \item \mnote{Observation: encoding format always is PBBBPBBB or PBBPBBPBB or PBPB; if we choose a representative frame in each sub-group, it is too many and agnostic to the semantic information. We try to construct a video representation compressing the video into a subset of frames while remaining the most information. PICTURE: compare the uniform sampling, DRL sampling, and Ours.} 
        \item Edge on residual/image/frame as a metric used in AccDecoder, SupreMo, FAST,\\ \underline{measures/decides the SR update} to overcome the ringing artifact from boundaries and texture in images. Reducto leverages Edge to measure the object detection results update; we use $\frac{1}{Area}$ 
        % \wnote{\sout{We need a metric to measure the Mask and/or inference updates. We may skip B frames and accumulate the residual of \underline{only P frames}, explore the }$\Delta Res(1,\cdots,7)\approx Res(1,4)+Res(4,7)$} 
        % \jnote{\sout{Shall we directly extract Edge feature on images? As we stood outside the decoder, we obtained all images.} Images have more information than residuals, which can make more accurate decisions on mask updates.}
    \end{itemize} 
    %                 \begin{figure}[h]
    %                 \centering
    %                 %\setlength{\abovecaptionskip}{1.2pt}
    %                 %\setlength{\belowcaptionskip}{0pt}
    %                 \includegraphics[height=2.0in]{figs/correlation.PNG}
    %                 \caption{Display order: Corr(Mask*, Edge-diff-on-residual) = 0.82. \wnote{Future TODO: improve the correlation to 0.9+. Solution\ding{172}: 1. decoding order; 2. accelerate raw residual. Solution\ding{173}: leverage the dependency graph. }}
    %                 \label{fig:StreamingCompare}
    %                 \end{figure}                 
                    %           
    \item Resource scheduling. Data need to be transmitted between CPU and GPU. \wnote{Shall we use CPU or GPU to decode?}
        \begin{itemize}
            \item If use GPU (AMD RX6000, RTX 30 LPT, RTX 30 DPT, RTX 40 DPT, RTX r4000) concurrent decoding and inference, are there any impacts? \mnote{Yes!! Put one Figure here.}
            \item How is the decoding performance of CPU (Intel, \sout{AMD}\wnote{AMD has no GPU on chip}) and GPU (RTX 30 LPT, RTX 30 DPT, RTX 40 DPT, RTX r4000) under various resolutions \& bitrates? \wnote{\ding{172}survey the HW architecture especially the CODEC chip first; \ding{173} characterize the GPUs to several categories.} \mnote{Yes!! Put one Figure here.}
            \item If 3D Mark can test the decoding performance only?
            \item To evaluate the latency, we can use average fps and 1\% low fps (to measure the kadun).
            \item The complexity of Canny edge detector O(HW*log(HW)), cost only 0.5ms on one 360P frame.
    \end{itemize}                 
\end{enumerate}

 
% \newpage

\wnote{\sout{We DON'T NEED SR reuse as it works \\ \underline{during decoding.} We dont want any "re-decoding" staff.}}

\wnote{FUTURE TODO: \sout{Residual occurred at the end of decoding of each frame. Shall we use some feature during the decoding of one frame? Such as dependency graph, MB's residual, or others?}}

% \textbf{Wat we have:} 
% \begin{enumerate}
%     \item all the decoded frames.
%     \item residuals
%     \item MVs
%     \item dependency.
% \end{enumerate}



% \begin{tcolorbox}
% \textbf{Given a video contains frame set ${\mathcal{F}}$, \ie macroblocks set ${\mathcal{MB}}$ where $Decode({\mathcal{MB}})={\mathcal{F}}$, select partial macroblocks $\mathcal{MB}_{s}$ to be enhanced such that average accuracy of this video is maximized:}
% \begin{equation}\label{equ:AccDecoder:problemFormulation}\small
% %\setlength{\abovedisplayskip}{3pt}
% %\setlength{\belowdisplayskip}{3pt}
% \begin{aligned}
% \textbf{(P1)}\quad max\quad &\frac{1}{|\mathcal{F}|}\sum_{i=1}^{|\mathcal{F}|} Acc_i(D(SR(\mathcal{MB}_{i})+\overline{\mathcal{MB}}_{i}), D(SR({F}_{i}))), \notag\\
% s.t.\quad &\mathcal{MB}_i\in\mathcal{MB}_{s}, t_{AVG} \leq 33ms, \notag
% \end{aligned}
% \end{equation}
% where, $\mathcal{MB}_i$ is the selected macroblock in frame $\mathcal{F}_i$, $\overline{\mathcal{MB}}_{i}=\mathcal{F}_i-\mathcal{MB}_i$. %$Hr({F}_{i})$ is the high-resolution version of frame ${F}_{i}$.
% \end{tcolorbox}

% We focus on the individual frames: key-portion-selection + SR + infer.
% Reuse the key-portion-selection results, \tb{reuse SR?}\wnote{NO! All of our work is out of decoder, \ie, we have already had the frames decoded in pixel domain}, reuse infer.

% \newpage

% \tb{LiveNAS} Our observation is that for videos with minimal scene change the online training gain eventually saturates to the point where further training may not provide benefit. However, video segments with frequent scene change benefit from continuous training. Thus, real-time adaptation to content can improve resource-efficiency.\\

% \tb{DDS} Moreover, unlike prior work that requires camera-side vision processing or hardware support (e.g., [30, 48, 80]), we only need standard video codec on the camera side.

% Challenge 2:

% Challenge 3: Make decisions about resource allocation before runtime; adjust allocation among streams at runtime.\\

% C3: System Overview

% C4: Region selector

\wnote{Picture here.} Figure illustrates our method beats previous methods, e.g., 3D-CNN, LSTM, and Transformer, in the form of speed. And use 1-3 sentences to analyze why they slow down the inference latency.

% C4.1: Spatial Selection - MB detection
% \begin{itemize}
%     \item Region selection -> MB-grained -> Optimization problem 
%     \item SS problem -> Loss function -> Model selection
%     \item Lightweight:
%     \item Compare to the hand-craft feature (edge-based [supremo, eagleeye]) and RPN ([DDS, better to follow]) it's much better.
% \end{itemize}

% C4.2: Temporal Selection - Frame selection
% \begin{itemize}
%     \item Mask change is not frequent. \wnote{Figure of Mask change in traffic video and on-board video}.
%     \item Leverage lightweight feature estimates the mask change and then selects frames. \wnote{Figure of the correlation ratio between $\frac{1}{OP_{area}}$ and $\Delta Mask*$}.
%     \item The CDF-based algorithm to sample frames.
% \end{itemize}

C5: Scheduler:

Cross-stream enhancer

HW determines processing capacity (including the batch size (or 3D patch shape) and the frames \#): PatchEnhancer measures the latency of modules once and allocates the number of anchors for each stream such that the total latency is less than the available computing time. \sout{Single stream - minimize latency for each chunk;} Multiple streams - maximize stream \# s.t. \jnote{the latency constrains.}
\ynote{Scheduling by chunk incurs an extra 1s latency/buffer in our E2E system. Parallel execution of the entire E2E flow of the 1st frame and other modules of the remaining frames, we can experiment with the longest processing delay among frames in one chunk.}
\begin{equation}\small
%\setlength{\abovedisplayskip}{-3pt}
%\setlength{\belowdisplayskip}{3pt}
    \max_{N} (\sum_{i=1}^N T_{pcs}(F[i])\leq T_{intv} * M)
\end{equation}
in most cases, $T_{pcs}$ equals to $T_{SR}$ that is the bottleneck of E2E system.
$T_{intv}$ is the time cost of processing a batch on a GPU. 


Priority: Sort the samples (or called anchor frames) in the global queue.

\wnote{Requirment:} Avoid data swaps between CPU and GPU as possible because the time cost is orders of magnitude larger than the computing time cost of DNN \mnote{(\eg, $100\times$ GPU to CPU at $3\times$ SR a 360*270*3 tensor)}.

C5.1: Patch + batch - 3-D patching. 
\begin{itemize}
    \item Batch \# subjects to the pipeline constraints (to avoid idle according to the synchronization).
    \item ALg: H\&W in the tensor shape fixed by the maximum patch, batch (C) is a variable to be determined.
    \item Change: Patch size \sout{per chunk} changes with content.
\end{itemize}

C5.1.1: Extension: 4-8 pixels to avoid patch error

C5.2: Task-Accelerator mapping/Placement
\begin{itemize}
    \item Variables: Single stream: \wnote{(Static?)} Task-Processor mapping
    \item CPU/GPU decoding latency comparison under 1080P, 2K, 4K video (Table).
    \item GPU Decode+Infer impact each other, and Memory I/O or PCIe result in latency and CPU idle (Figure Appendix).
    \item CPU inference ability with OpenVINO works well (\wnote{?}).
    \item Multi-threading or single-threading (\wnote{add an experiment shows batching vs load multiple models, which is better}).
    \item Sequential execution on GPU, not Parallelism, because \ding{172} GPU utilization is almost 99\% with batching, \ding{173} each instance will occupy more than 1G GPU extra memory by Pytorch. 
    \item NeuroScaler does not work in our scenario. The video consists of frequent-change scenes generating the amount of key frames, \eg, one of every 14 frames in Auto-driving [BDD], incurs too much computing cost.
\end{itemize}





% \sout{C4: Scalability and Optimization}

% \sout{C4.1 Multiple streams}


% C6: Additional Optimization

% C6.1: Integrated with enhancement reuse

% [Nemo, Neroscaler, AccDecoder]

% C6.2: Integrated with inference results reuse

% [EAAR, AccDecoder, MobiPose] 


% \newpage

\subsection{How to reuse the }
1. how to select frames to minimize the loss in real time?

1.1 how to handle the order difference between decode and display? Almost the same. No big deal.

2. how to face various selected requirement of different computer vision tasks? 

3. how to handle online training? When to start and when to end?


% \subsection{Intra-frame SR}

%%
% \textbf{Observation:} SR improves \textasciitilde10\% confidence of true positive object and decreases \textasciitilde10\% of true negative object.

% %%
% \tb{Approach:} 1. execute SR on RPN output which are \textasciitilde$\pm$10\% around confidence threshold.
% %
% 2. should contain the context information [SOD-MTGAN: Small Object Detection via MultiTask Generative Adversarial Network. In ECCV, 2018.][SR for Small OD]
% %

% \cb{RPN [DDS, Better to follow] Or edge-based background [Eagleeye, SupreMo] filter? Shall we add an experiment to clear compare them by latency and accuracy?}

% %%
% \tb{New Challenge:} Previous SR aims to improve PSNR, thus dividing frames into slices for parallelism does not reduce SR's enhancement. 
% %
% While, to object detection, dividing one object into several slices will significant harm SR's enhancement. 
% %
% current work: [ELF, Mobicom'21] is too heavy for streaming application.


%%
% \subsection{Inter-frame SR: How to select frames?}
% %
% In experiment, we find that when a frame is up-scaled using cached high-resolution frames, inference accuracy degradation inevitably occurs.
% %
% For example, the inference accuracy drops drastically when only upscale I-frames.

% %%
% how does video decoder work (2.2 in Compressed video action recognition is good-writing).
% %
% \cb{Motion vector image use HSV space, residual image use absolute RGB is better.}

%%
% \textbf{Observation:} 

%%
% \tb{\cb{Reuse error:}} experimental results illustrates bicubic brings accuracy loss.

% \cb{Difference:} NEMO's search algorithm is too heavy for streaming case, and its consideration aim to tackle scene change frequency case which significantly differs from continues traffic/auto-driving case.

% %%
% \tb{Approach:} We try to use \cb{low-level features operate on residual} to find out the reset point.
% %


% %%
% SR transferring is for detecting on un-SR frames.

% video ingestion order \vs encoding order 

%%
%\tb{To reduce computation cost \& inference latency.}
%
%These two goals commonly share the same methods. %because the inference time is decreased at the same time when reduce the computation cost. 
%
\hide{
%\vspace{-1.5em}
\section{Introduction}
%%

%%
In this context, we bring holistic thinking of video codec and inference tasks into VAPs. %; this reveals new opportunities to increase accuracy and decrease latency. 
The fundament of video encoding is using signal processing techniques to eliminate \emph{block-level} (a small region contains $16\times8$ or $8\times8$ pixels in frame, see \ref{subsec:Background_encoding} for details) spatial-temporal redundancies on that occur in videos; coincidentally, distributed VAPs transmit video from the camera to the edge/cloud for compute-intensive inference, which naturally necessitates video encoding and decoding. 
Bits stream (the data format of compressed video stream in distributed VAPs) contains plenty of free information about key blocks can help us find out the ``important'' content. 
On the other hand, how video encoding eliminates spatial and temporal redundancies hidden in the bits stream can accelerate the ``important'' content enhancement and inference. 

%%
The challenge of subframe-enhancement mechanism, however, is \emph{how to derive important content and enhance them from free block-based bits stream.}
To demonstrate the feasibility of the approach, we prototype the system and quantify benefits and cost of it.
We open the decoder and take a first attempt to answer the following question: \emph{How overlooked but handy information in decoder helps accelerate and improve video analytics system?}
In answering this question, we dig out and make use of frame also macro block dependency from decoder.
We believe that there is still many information unexplored to achieve larger improvement (see \S \ref{AccDecoder_sec-newResDire}).


%%
%Heterogeneous quality assignment in frame has already proposed in non-enhancement-participated VAPs design \cite{du_server-driven_2020, meddeb_region--interest-based_nodate ,liu_edge_2019, xie_source_2019, du_AccMPEG_2022}, however, they inevitably fall into the assumption of frame-level processing.
%
%They 



%%
Video encoding; it first divides the entire frame into macro blocks, then captures both spatial and temporal redundancy among them. 
%
Temporal redundancy, occupying a dominant position in video redundancy, represents similarities between successive frames; to compress it, inter-frame coding encodes the difference between adjacent frames to compresses a motion picture.
%
DNN inference model learns high-level features from a complex low level representation of data; it abstracts semantical meaningful features from images.
%
Obviously, here is a gap between encoding and DNN model, however, our key intuition is that \emph{the encoding information (\eg, reference frame and motion vector), while not accurate, is sufficient to reveal what information can be reused, thereby speed up SR enhancement (see \S \ref{sub:SR}) and DNN inference (see \ref{sub:mv})}.
%%
%\emph{However, we are on the side of enhancing only important partial content in partial frames}.
}



%%%
%Accordingly, we design a content-aware DNN-integrated video decoder utilizing (not repeated computing) encoding information to find out ``right'' frames/pixels.
%In particular, our design explores the relationship among encoding, low-level image features, and semantic features to exploit ``important'' content; and leverages redundant information to reuse the intermediate or final DNN results of these frames/pixels for inference acceleration.


==> KeyDesignChoices.tex <==
\section{Key Design Choices}
To overcome the limitations of frame-level enhancement in \ref{subsec:PotentialGain}.
AccDecoder applies enhancement (SR) only to partial ``important'' content in a subset of frames and transfer them to the remaining frames; it also applies inference DNN only on a subset of frames and transfer the inference results to other frames.
The goal is to amortize the computational overhead of a SR DNN across the video.
Moreover, we want to provide a guarantee that the resulting inference accuracy within a small margin compared to the per-frame enhance and infer; at the same time, guarantee the whole mechanism subject to the real-time constraint.
We ask ourselves a series of pivotal questions that lead to the key design choices we make in achieving the goal.

%%
\subsection{On which granularity in bits stream to find out ``important'' content for enhancement?}
%
\tb{Key Observations.} ``Important'' content is the image after enhancement may improve the inference accuracy. 
Recent studies from computer vision community (\eg,\cite{Noh2019Better}) and networking community (\eg, \cite{wang_enabling_nodate, du_server-driven_2020}) find that the enhancement perfectly improve the inference results of small objects (\eg, the size of traffic signs in Tsinghua-Tencent 100K dataset \cite{zhu2016traffic} are only $32\times32$ pixels but occupy $42\%$ total number of objects).
Coincidentally, \emph{macroblock (MB)} is the quantization parameter (QP) assignment unit in video codec to determine the image quality of this $16\times16$-pixel content.
On macroblock-grained, it is not too fine-grained (compared to pixels) to build huge solution space for searching important content, and also not too coarse-grained (compared to frame) to waste computational resource for enhancing unimportant content.

%%
\tb{Approach.} 
%
AccDecoder applies enhancement only to a subset of MBs, referred to as \emph{anchor MBs}.
The remaining MBs reuse the enhanced MBs according to the block dependencies (See Sec. \ref{subsubsec:reuse}) to up-scale their resolutions.
Because enhancement models \cite{Hui_2018_CVPR, ahn2018fast, 8014885} often use overlapping blocks to extract frequent information, AccDecoder expands each anchor MB to each direction by $\beta$ blocks (if they are not already selected).
At the same time, to match the rectangle image shape feeding into enhancement model, AccDecoder fills the holes by switch the unselected blocks to selected one.

%%
\subsection{What to Reuse and How?}\label{subsubsec:reuse}
%
%\subsubsection{Enhanced MB reuse}
\tb{What to reuse.} To make the most out of caching, we \emph{cache the final output} (\ie, the enhanced high-resolution image) follows the same idea in \cite{yeo_nemo_2020, zhang_fast_2017}.
Their results show most of the latency occurs at the last couple of layers which means caching and reusing the output of enhancement model (\eg, SR model) is the most effective in computation reduction.

% %
% \begin{figure}[h]
% \centering
% \includegraphics[height=1.4in]{figs/InterFrameDecodeing.pdf}
% \caption{Illustration of inter-frame decoding. Block dependencies in decoder present an implication to reuse.}
% \label{fig:InterframeDecoding}
% \end{figure}
%

%%
\tb{How to reuse.} Inter-frame encoding in common codecs (\eg, H.26x \cite{H.264, H.265} and VPx \cite{VPx}) leverages temporal redundancy among frames (in a group of picture) to ``reuse'' similar regions from reference frames.
Figure \ref{fig:InterframeDecoding} illustrates the process of decoder decoding an inter-coded block with dependency information.
Decoder first uses reference index to extract a reference frame from previous decoded frames; then, it applies motion vector to the source block in the reference frame to transfer the block to the target frame; at last, it adds residual to the the transferred block to recover the target frame.
Inter-frame dependencies allow us to enhance only some MBs, but reuse these enhanced MBs to reconstruct others.


\hide{
\tb{Challenge and Intuition.} Via further analysis, we observe that the root cause of the accuracy degradation is the new appeared objects not being up-scaled.
%
For example, Figure \ref{fig:NewAppearedObj} shows a white car appeared at right bottom corner.
%
Based on our experiment results, if this frame is not up-scaled via SR model and thus the car cannot be detected by inference model, it also can't be detected in the following frames which are reused this SR frame.
%
Fortunately, we observe that with the new object appeared I-blocks also gather together among new appeared object as shown in Figure \ref{fig:IblockDistri}.
%
The reason is I-block using intra-frame coding which only uses the pixels in this block to compression; new appeared objects, obviously, can't refer to other frames.
%
In the future work, we try to leverage the distribution information of I-blocks to select frames to be up-scaled.
}

%Analyzer +RPN (optional) +DNN-driven SR +Controller

% \begin{figure}[h]
% \centering
% %\begin{minipage}[t]{0.28\linewidth}
% %\centering
% %\includegraphics[width=1.90in]{chapters/AccDecoder/figs/framet.png}
% %\subcaption{Object detection results (yellow bounding box) in $t$-th frame.}
% %\label{fig:ODonframet}
% %\end{minipage}
% %\hfill
% \begin{minipage}{1\linewidth}
% \centering
% \includegraphics[height=1.7in]{figs/MotionVector.png}
% \subcaption{Motion vector between $t$-th frame and $t+1$-th frame.}
% \label{fig:MotionVector}
% \end{minipage}
% \begin{minipage}{1\linewidth}
% \centering
% \includegraphics[height=1.7in]{figs/framet+1.png}
% \subcaption{Object detection results. Yellow boxes are from $t$-th frame, red one from $t+1$-th frame.}
% \label{fig:RelationofMV&OD}
% \end{minipage}
% \caption{The motion vector implies the movement of bounding box and the static region in image}
% \label{fig:MVimplication}
% \end{figure}

%%
\subsubsection{Additional Inference result reuse}\label{sub:mv}
\tb{How to reuse.} Motion vector indicates the offset of pixels among blocks in target frame and reference frame.
Although pixel-level offset is very difficult mapping to semantic meaning (\eg, object) in object \cite{10.1145/3152434.3152440}, we argue that motion vector provides enough information to speed up inference without compromising accuracy especially in static traffic or surveillance cameras.
Figure \ref{fig:MVimplication} shows the relation between motion vector and bounding box (Bbox) of detected objects.
From this relation, we have two observations to speed up inference.
Figure \ref{fig:MotionVector} illustrates the motion vectors between $t$-th frame and $t+1$-th frame; \ref{fig:RelationofMV&OD} shows the inference results of object detection on both $t$-th and $t+1$-th frame.

%%
\tb{What to reuse in Object Detection.} From the enlarged image of white moving car, we observe that the motion vectors of object always gather together and perfect match the movement of objects' Bboxes.
Accordingly, VAP does not necessarily execute object detection on current frame but instead move the Bboxes of the reference frame along with the motion vector of each object; then, its inference latency gets amortized with the reference frame.
We find that accuracy of motion vector decreases as the scene varies drastically, but taking a pragmatic stance to focus on static cameras, the performance has been  maintained high lever.

%%
\tb{What to reuse in Semantic Segmentation.} To some other CV applications, like semantic segmentation whose output is the class of each pixel, reuse the output of reference frames is not practical.
However, the motion vector also presents an opportunity to reuse intermediate results of inference model.
We observe that macro blocks with small motion vectors often has similar pixel values.
Follows this observation, we can cache the feature map (\ie, output of convolutional layer) of these macro blocks in reference frame and load them when execute convolution on the current frame.
%%
\subsection{How to Guarantee Performance?}\label{subsubsec:selection}
%
\tb{Key Observations.} We would like to ensure that the accuracy performance AccDecoder delivers is within a small margin (\eg, $\leq 0.1$ f1-score) compare to that of per-frame enhancement while the constraint of the average latency (from receiving the bit streams to rendering the inference results on each frame) is no more than $33$ms (\ie, $30$fps).




%To measure the benefit of reuse, we build a decoder which integrates our pre-trained task-driven SR model.
%
%\cb{Figure \ref{fig:FrameReuse} plots the the inference accuracy varies with the number of up-scaled frames.

%%
\tb{Approach.} We view it as two-level optimization problem that the upper-level frame selection problem categorizes all frames into three classes -- SR frames, detect frames, reuse frames; the lower-level anchor MBs selection occurs on the select frames belong to SR class.
Obviously, there is a gap between our approach and optimal solution of \textbf{P1} and we are focusing this gap when I am writing this dissertation. Hope we have good results.

%%
\noindent\emph{Select anchor MBs in SR frames.} We use AccModel, proposed in \cite{du_AccMPEG_2022}, to measure how sensitive of the quality change of macroblocks ($16\times16$ pixels region) in one frame to the accuracy. 
AccModel is a light-weighted DNN (MobileNet-SDD \cite{howard2017mobilenets} append three convolution layers).
It maps a frame into a matrix that each element is the sensitivity value of the macroblock at the corresponding position.
The sensitivity of the very top left $16\times16$ pixels, for instance, corresponds to the column-one-row-one element in the matrix.
%The reason for using macroblock, not frame or block, as the measurement unit is that it is the quality assignment unit in video codec (\eg, H.26x, VPx).
%views macroblock quality assignment as a segmentation task, in which it leverages a
Fig. \ref{fig:AccModel} visualizes the matrix values in the $4$-th frame in dataset \cite{TrafficCam2}, in which the small object (\eg, the cars in the top half frame) is sensitive to quality change, namely, these macroblocks should be enhanced. 

%%
\noindent\emph{Categorize all frames into three classes and their execution pipelines.} For each frame in SR class, selected anchor MBs are enhanced by SR model and the remaining MBs are bicubic interpolated; after this, feeds the up-scaling frame into final DNN (\eg, object detection) for inference. 
To the frames in detect class, they earn the benefits from SR MBs following the dependencies in Fig. \ref{fig:InterframeDecoding} then feeds into final DNN for inference.
Their accuracy still increases a lot due to the benefits transferring from SR MBs.
Note that the transferring is quite fast (the time cost is the same as normal frame decoding) as it only includes additional bicubic interpolation on residual per frame compared to normal frame decoding.
To those frames in reuse class, \eg object detection, we get the bounding box of each object in the last (playback order) detect frame, calculate the mean of all motion vectors that reside in the bounding box, and use it to shift the old position to the current position.
While, to the semantic segmentation for reuse frames, we get the class of each pixel in the last (playback order) detect frame, calculate the mean of all motion vectors for each macroblock, and use it to determine whether the pixels in this macroblock is static (compared to last detect frame) or not; if it is static, then set all pixels in this macroblock black. 

%%
\begin{figure}[h]
\centering
\includegraphics[width=2.4in]{figs/mvuse.pdf}
\caption{Reuse error accumulation of MVs}
\label{fig:MV_accuracy}
\end{figure}

%%
\noindent\emph{Categorize metrics.} The accuracy of reuse frames drop dramatically along with error accumulation from cache of SR MBs or inference results. 
In Fig. \ref{fig:MV_accuracy}, taking Object Detection as an instance, reusing bounding box detected in the first frame to the following frames causes significant accuracy reduction.
Consequently, \emph{we should carefully categorize three classes.}

%\begin{figure}[h]
%\centering
%\includegraphics[width=2.4in]{chapters/AccDecoder/figs/resimg.pdf}
%\caption{Correlation between differencing values of Laplacian on both image and residual and changes in Bbox results}
%\label{fig:correlation}
%\end{figure}


The constraint of real-time ($30$fps) video analytics restricts us not to use heavy-weighted metrics to categorize frames. 
Here, we extract the light-weighted features on the residual of each frame. 
Our intuition is information of residual is sparse and de-redundent.
It preserves difference among frames but not too dense to process, thus provides us a good opportunity to efficient filtering frames for free.
We tried many light-weighted features (\eg, Pixel, Edge, Area, HoG used in \cite{li_reducto_2020}) and find out the Laplacian (\ie, Edge) on residual has a high correlation with the inference accuracy.
Fig. \ref{fig:correlation} plots the correlation is very strong which implies that Laplacian on residual profiles the impacts of reuse error very well.
At the same time, executing Laplacian operator on residual is $34\%$ faster than that on image as Fig. \ref{fig:resspeed}.

%%
%\begin{figure}[h]
%\centering
%\includegraphics[width=2.2in]{chapters/AccDecoder/figs/resspeed.pdf}
%\caption{Time comparison of executing Laplacian on residual and image}
%\label{fig:resspeed}
%\end{figure}


==> Motivation.tex <==
\section{Background}
We start with setting up the basic knowledge (\S\ref{subsec:Background}) then its status quo (\S\ref{subsec:Statusquo}).

%%
\subsection{Preliminary knownledge}\label{subsec:Background}
%P1: Briefly introduce the current state of video analytics from the amount of industry.
%P1: Tasks of video analytics. 
\tb{Video Analytics Pipeline (VAP).}
Many computer vision tasks are considered in VAPs, such as traffic control \cite{Ganesh_Real_2017}, surveillance and security \cite{yi_eagleeye_2020, liu_caesar_2019}, as well as digital assistant \cite{Siri}.
%
We consider two tasks as running examples --\emph{object detection} and \emph{semantic segmentation}.
%
Object detection aims to identify objects of interests (\ie, their locations and classes) on each frame in the video, whereas semantic segmentation labels each pixel with one class.
%
Selecting these two tasks has two major reasons: first, both of them play the core role in computer vision community because a wide range of high-level tasks (\eg, autonomous driving) are built on them; second, we seek to keep consistent with prior video analytics work \cite{jiang_chameleon_2018, du_server-driven_2020} to let the performance comparison be more straightforward and convincing.


%% 
%P2: (Topic: Discuss video streaming in video analytics). 
%
\tb{Distributed Architecture.}
The proliferation of VA is facilitated by the advances of deep learning and the low prices of high-resolution network-connected cameras. %computation unit (\eg, GPU).
%
%-> Explain why we need stream video to Edge/Cloud 
However, the accuracy improvement from deep learning is at the high computational cost. 
%
Although the state-of-the-art smart cameras can support deep learning method, the deployed surveillance and traffic camera paint a much bleaker resource picture.
%
For example, DNNCam \cite{DNNCam} that ships with a high-end embedded NVIDIA TX2 GPU \cite{NVIDEA_TX2} costs more than \$2000 while the price of deployed traffic cameras today ranges \$40-\$200 \cite{WyzeCamera, Trafficcamera}; these cameras typically loaded with a single-core CPU only provide very scarce compute resource\footnote{Professional UAVs may equipped with high-end GPUs but most of civilian UAVs are not}.
%
%-> State the workflow (how) of such distributed video analytics. 
Because of this huge gap, the typical \emph{video analytics pipeline (VAP) follows the distributed architecture}. 
%
\emph{E.g.}, a vehicle detection pipeline consists of: a front-end traffic camera compresses and streams live video to a compute-powerful edge/cloud GPU server upon wire/wireless network; and, a back-end server decodes received video into frames and feeds them into models (\eg, Faster RCNN \cite{conf/nips/RenHGS15}) to detect vehicles.
%
%(-> How to cope with bandwidth fluctuations) not necessary I think.

%%
%P3: (Topic: Discuss distinctive feature/aim of video analytics: tradeoff among bandwidth cost \& accuracy \& latency)

\tb{Video codec basics.}\label{subsec:Background_encoding} 
Video codecs, composed of encoder and decoder, are software/hardware program used to compress size of video files for easier storage or delivery over network. 
Encoders compress video data and wrap them into common video formats (\eg, H.26x \cite{H.264}, VPx \cite{Webm_offical}, AVx \cite{AV1}), while decoders decompress the compressed video data into frames before post-process (\eg, playback or analysis). 
By selecting the encoder, its coding standard and algorithm will determine the computational cost and compression effect. 
For example, MPEG4 encoders usually have low hardware requirements and are easy to implement, while H.264 ones have better compression. 
This compression process is usually lossy, which strikes the balance between video quality and compression ratio according to encoding settings of users (\eg, bitrate, frame rate, and group of pictures).



%The compression ratio and video quality depend on codec itself and encoding settings. 
%By selecting codec and adjusting the encoding settings, one can strike balance between quality and compression ratio.
Let us taking H.264, one of the most popular codecs, as an example explain the compression process.
During encoding, each video frame is first divided into non-overlapped macroblocks ($16\times16$ pixels), then to each macroblock, the encoder searches for the optimal compression method (including the block division types and encoding types of each block) according to the pixel-level similarity and encoding settings. 
One macroblock may be further divided into non-overlapped blocks ($8\times8$ or $8\times16$ pixels) and each of them is encoded with intra- or inter-frame types. 
The intra-coded block is encoded with the most pixel-value similar reference block in the same frame, and the offsets between these two blocks are encoded into \emph{motion vector (MV)} and \emph{residual}.
With the same procedure, inter-coded block locate the most pixel-value similar block searched by reference index and motion vector from other frames.
Motion vector indicates the spatial offset between the target block and its reference while the difference in pixel values of two blocks is encoded as residual for decoding\footnote{Conceptually, \{target block\}$=($\{reference block\}$+$\{residual\}$)\cdot$\{MV\} (here we represent the MV as a matrix).}. 


%%
\tb{Performance metrics.} Under this distributed architecture, the focal point of VAP is the tradeoff among three performance metrics: \emph{accuracy}, \emph{resource (bandwidth \& computation) cost}, and \emph{latency}.

%%
%Definition of Accuracy + Definition of bandwidth cost + Definition of latency.
\begin{itemize}
	\item \emph{Accuracy.} %\cb{Instead of evaluating performance of VAPs in the context of a particular application, this work focuses on the relative accuracy improvement from AccDecoder: 
	We comparing output on each compressed frame of this VAP %in the streamed compressed video 
(under limited bandwidth) with the output of the state-of-the-art analytics model on the same raw frame%but from uncompressed (highest quality) video
\footnote{Raw frames often encodes into video with quality loss by setting quantization parameter (QP). The larger QP value, the smaller video file size but lower quality. Here, we define highest quality video when setting QP as 0.}. 
	%
	Using the output of this \emph{golden configuration}, the state-of-the-art model and raw video input, instead of human-annotated labels as \emph{``ground truth''} is useful in real applications and consistent with recent works \cite{jiang_chameleon_2018, zhang_live_nodate, zhang_awstream_2018}. 
	%
	This way, any inaccuracy will be due to VAP designs (\eg, video compression, DNN itself).
	%
	We identify \emph{F1 score} as metric in objects detection task (the harmonic mean of precision and recall for detected objects' location and classes) and %\cb{\emph{IoU}} in 
	semantic segmentation (the intersection over union of pixels associated to the same class).
\item \emph{Resource (Bandwidth \& Computation) cost.} We define the total size of the video file delivered from the camera to the server of each VAP as its bandwidth cost. As GPU is the major hardware running DNN today, we use GPU time ($100\%$ usage ratio) to measure the computation cost of VAPs.
\item \emph{Latency.} In general, the end-to-end latency is the time interval from the time of camera capturing one image to the model on sever outputs its inference result, which consists of the camera processing (capturing images and encoding them into video) time, video delivering time, and server processing (decoding video into frames and run inference on each of them) time.
	%
	In this paper, we focus on designing a tool (\emph{AccDecoder}) which can plug into the server of any VAPs to accelerate the inference, thus we measure the latency includes the video delivering time and server processing time.
\end{itemize}

%%
\subsection{Video analytics pipeline: status quo}\label{subsec:Statusquo}
%%
Here, we categorize the status quo of video analytics pipelines in four classes and analyze their limitation on purchasing \emph{high accuracy, low resource cost}, and \emph{low latency}.


%%
\tb{Server-training camera-executing video compression.} 
Pioneer methods \cite{xie_source_2019, du_AccMPEG_2022} divide the VAPs into two stages: offline training and online executing.
\cite{xie_source_2019}, on server, periodically probes inference DNN with accumulated images in time slot and search the best assignment for the weights of YUV channels; the broadcast the results to all cameras for encoding images in the next slot.
\cite{du_AccMPEG_2022}, trains a shallow DNN which can assign high-or-low quality for all macroblocks (a small region containing 16$\times$16-pixel image) in a frame on server; then deploy this DNN on camera to assign qualities for encoder.
% Server earch and assign the best values of parameters for image or video encoder on camera. 
%(\eg, MPEG and H.264 in ) driven by DNN on server and historical content, therefore, their decision lags current image content.

%%
\tb{Server-side data enhancement.} %Data enhancement improve users' quality of experience via a learning DNN model (\eg, Super Resolution (SR) \cite{} or Generative Adversarial Networks (GAN) \cite{}) upsampling low-resolution images to high-resolution ones. %then feed them into inference model.
%
Inspired by their succeed of image enhancement (via Super Resolution (SR) \cite{Hui_2018_CVPR, ahn2018fast, 8014885} or Generative Adversarial Networks (GAN) \cite{Chen_2018_CVPR, NIPS2017_892c3b1c}) in video streaming for human-centric quality of experience (\eg, \cite{yeo_neural_nodate} and \cite{yeo_nemo_2020} considers video on demand, \cite{kim_neural-enhanced_2020} works for live video streaming), some studies \cite{wang_enabling_nodate, wang_bridging_nodate, yi_eagleeye_2020} expand this approach to  machine-centric video analytics system. %to increase accuracy
%
It indeed increases accuracy, although, as we will elaborate in \S \ref{subsec:limitation}, the latency it causes much offset the accuracy increasing.
%
The root cause is that image enhancement models are much heavier than other computer vision models. 
%
For instance, the complexity of SR model is as high as $1000\times$ heavier than image classification and object detection model in terms of MultAdds \cite{yi_supremo_2020}. %as SR output HR images whereas others output labels or bounding boxes.

%otherwise, low-quality video will cause false labels (compare to golden configuration), which results in retraining restricted accuracy of student model \cb{(add one figure (\& one snapshot) to plot the 520P/270P on resnet101 and the 1080p)}. 

%%
In our system, we take a pragmatic stance to focus on the backend (edge/sever) in the design space -- \emph{decoder}. 
With no camera-side processing, no server-driven, and no model retraining, only data enhancement, we systematically exploits the abundant information in bits stream to improve enhancement mechanism. 
The reason is that: first, as we discussed in \S \ref{subsec:Background}, majority of installed surveillance or traffic cameras only equipped with cheap CPU, which cannot support SOTA camera-side analytics-aware video compression method.
Second, decoder plays the pioneer role for analyzing the bits stream.



%the very beginning module on edge/server

%no camera-side frame-dropping heuristics, no model distillation (use the server-side DNN as-is), and no change to the video codec; instead, we use the server-side DNN output to drive spatial quality adaptation.


%Two categories concerned in VAP design to increase accuracy are: \emph{improve the quality of data} and \emph{improve the performance of model}.
%
 
%
%Another way to improve data quality is video encoding optimization.
%

%%
%\tb{To decrease bandwidth cost.} The core thinking here is \emph{mitigating video feed into network}.
%
%Adapt the configurations (\eg, the resolution and the frame rate \cite{jiang_chameleon_2018, zhang_awstream_2018}) or discard frames containing only worthless information (\eg, static video content \cite{chen_glimpse_2015, hsieh_focus_18, kang_noscope_2017}) for the temporal variance of video content, and encode each frame with a spatial uneven quality distribution (\eg, high quality for pixels in the region of interest, such as target object, but low quality for the background \cite{du_server-driven_2020, liu_edge_2019, meddeb_region--interest-based_nodate}) to tackle the spatial variance in each frame, all mitigate the video feed into network. %in order to avoid wasting bandwidth onalso saves bandwidth usage.
%
%As we will elaborate in \S , image enhancement, although, indeed increase accuracy, the latency it causes much offset the accuracy increasing.
%
%Mitigating data feed (bandwidth): frame/region filtering with local classifier/guided by backend <> limitation: local classifier incurs accuracy drop \& backend guidance cause more latency.

%
%Bandwidth saving. First, since the camera can access raw video, they can use their own compute power \cite{chen_glimpse_2015, liu_edge_2019, kang_noscope_2017} or guided by cloud's feedback \cite{jiang_chameleon_2018, zhang_awstream_2018, du_server-driven_2020} to discard frames containing worthless information (from temporal dimension); these frames won't be delivered to the cloud hence save bandwidth cost. Second, in video streaming system, information of interest (\eg, target objects) are sparsely distributed in each frame, streaming only the region of interest (from spatial dimension) \cite{zhang_design_2015, hsieh_focus_18} also save bandwidth cost.  

%%



%
%frame filtering studies \cite{chen_glimpse_2015, li_reducto_2020} in decreasing bandwidth cost can also be thinking of a type of tracker method (They reuse the inference results from the previous nearest frame).

%%
%\cite{hsieh_focus_18, kang_noscope_2017}

%%

%%
%\tb{Limitation of existing pipelines.} 
%
%The place where decision making to decrease bandwidth cost categorizes into: camera-side cheap decision making and server-side close-loop control.
%






%%
%\tb{Limitations of conventional video analytics pipeline.} Although current bandwidth saving and accuracy increasing approaches have served us well, there are still three significant limitations.
%
%\vspace{-0.5em}
%\begin{enumerate}%[itemsep=-4pt, topsep=3pt, leftmargin=18pt]
  %\item \emph{Camera-side decision making reduce inference accuracy while server-side decision making increase latency.}  Camera -side decision making leverages  \cite{zhang_design_2015} or heuristic method (\eg, inter-frame pixel-level difference \cite{chen_glimpse_2015}) to distinguish and prune frames/regions without valid information. However, these cheap methods may cause false positive (\eg, pixel-level distance changes by background may trigger camera to send many frames) and false negative (\eg, small appeared objects may be missed by cheap object detection model), thus increase bandwidth cost or reduce the inference accuracy. Server-side decision making control camera's actions with feedback from cloud. For example, the camera in \cite{du_server-driven_2020} iteratively delivers the region of interest with higher resolution follow the feedback from cloud. Obviously, this sever-side decision making (\ie, a closed loop control mode) introduce extra latency especially delivery between camera and cloud cross wide area network.
 %
%Camera configuration with low resolution and frame rate cause deterministic hurt to small object (\cb{learn how to describe from ASR}).
% 
  %\item \emph{Image enhancement contribute higher accuracy but also cause higher latency.} Although recent studies achieve great success in leveraging image enhancement for increase QoE and inference accuracy, they still suffer from high latency. 
 %Although this approach brings higher inference accuracy, it relies critically on the client's computational capacity. heavily depends on the network condition -> Enhanced images increase accuracy, and not limited by network condition.
%
%Mobile \cite{lee_mobisr_2019, yi_eagleeye_2020, yi_supremo_2020}, Even with desktop-class GPUs \cite{wang_bridging_nodate, wang_enabling_nodate}, which real-time streaming cannot achieve. 
%
  %\item \emph{Computer vision community and networking community both neglect existing information in decoder.} Computer vision community treat CV tasks on video as an algorithm/model design problem, researchers focus on presenting novel and general models; accordingly and naturally, their studies are short of systematic consideration from video analytics applications. Studies in networking community reveals the strengths (\eg, increase accuracy) and weaknesses (\eg, feed amount of data into wide area network) of distributed VAPs. However, all VAPs do not make full use of video encoding information; many of them \cite{chen_glimpse_2015, liu_edge_2019, zhang_mobipose_2020} borrow the idea of video encoding designing their frame filtering mechanism and executing on the frames outputted from the decoder, thus introduce extra latency. The root reason is that prior studies separately design every component rather than holistic consider entire VAP system, and thus neglect information in hand. 
%\end{enumerate}


%most of the installed surveillance or traffic cameras only embedded cheap CPU which are unable to support DNN execution; some of them even cannot be programmable.

%%
\section{Motivation}
In this section, we elucidate the pros and cons from enhancement (\S\ref{subsec:limitation}) and use empirical measurements to illustrate the potential improvement (\S\ref{subsec:PotentialGain}).

\subsection{Pros and Cons from Enhancement}\label{subsec:limitation}
%%
\tb{Pro: Accuracy Increment.} 
%
Existing studies has shown enhancement improves the task accuracy a lot; \eg, in object detection, image enhancement in \cite{wang_enabling_nodate} improves the $4\%$ accuracy while enhance only small objects mechanism in \cite{Noh2019Better} improves the accuracy of small objects up to $9\%$.
We preliminary study the accuracy improvement by image enhancement.
%The experiment platform is the same as \cb{Sec. \ref{}.}
We compare the results from original resolution video with $320\times180$ resolution (lr) to SR video with three upscaling factors $2\times$ (to $640\times360$ res), $3\times$ (to $960\times540$ res), and $4\times$ (to $1280\times720$ res).
As the upscaling factor increases, the accuracy also increases but the accuracy gain emerge diminishing marginal utility; in particular, compared to lr, $2\times$ increase $7\%$ average accuracy, while the benefit of $3\times$ and $4\times$ is diminishing.

\begin{figure}[h]
\centering
%\setlength{\abovecaptionskip}{1.2pt}
%\setlength{\belowcaptionskip}{0pt}
\includegraphics[height=2.0in]{figs/StreamingCompare.pdf}
\caption{Streaming Protocol Comparison}
\label{fig:StreamingCompare}
\end{figure}
%%
\tb{Pro: Bandwidth Save.} 
Video streaming in analytics pipeline is sensitive to the variation in available network bandwidth.
Fig. \ref{fig:StreamingCompare} shows the the available bandwidth and video bitrate for video streaming for analytics (here use DDS \cite{du_server-driven_2020} as an example), compared with live video using WebRTC for user viewing and on-demand video using adaptive streaming (DASH) \cite{yuan2022VSiM, dash} given a FCC broadband network trace \cite{FCC}.
Video streaming for analytics, comparing to WebRTC, uses bandwidth more aggressively by sharply adjusting the encoding quality (\eg, quantization parameter, qp, in \cite{du_server-driven_2020, zhang_awstream_2018}) because it does not need to smooth the quality of successive chunks (2-10 second video) like WebRTC does for better user quality of experience.
However, compared with on-demand video streaming, two live video streaming use bandwidth much more conservatively.
The root cause is that %1) large buffer of on-demand video streaming effectively absorbs bandwidth variations; and 2) 
pre-encode chunks with various bitrates in on-demand video streaming provide the chance to probe and retransmit the same-content but different-bitrate chunk.
As a result, the bandwidth utilization of video streaming in analytics is pretty well, but the backend of VAPs still has plenty room to explore. %it is  WebRTC requires much larger bandwidth than adaptive streaming clients for the same quality.

% \begin{figure}[h]
% \centering
% %\setlength{\abovecaptionskip}{1.2pt}
% %\setlength{\belowcaptionskip}{0pt}
% \includegraphics[height=1.4in]{figs/BandwidthSaving.pdf}
% \caption{Bandwidth Saving}
% \label{fig:BandwidthSaving}
% \end{figure}

%%
In backend, enhancement can significantly improve accuracy without requiring more bandwidth.
Fig. \ref{fig:BandwidthSaving} plots the bandwidth usage of enhancement mechanism (frontend transmits low-resolution video then backend enhances into high-resolution one) and two state-of-the-art VAPs (\ie, DDS \cite{du_server-driven_2020} and Reducto \cite{li_reducto_2020}) under the same target accuracy.
The frontend in baseline directly transmits all high-resolution frames as a benchmark.
DDS iteratively transmits low-resolution video and partial high-resolution video while Reducto only transmits necessary frames. 
In figure, enhancement mechanism only cost near half bandwidth of DDS and one third of Reducto, which demonstrates enhancement-participated mechanism saves considerable bandwidth compared to server-driven video compression (\eg, DDS) and camera-side analytics-aware video compression (\eg, Reducto).

%%
% \begin{figure}[h]
% \centering
% \includegraphics[height=2.2in]{figs/Latency.pdf}
% \caption{Latency Break Down}
% \label{fig:AccuracyLatency}
% \end{figure}

%%
\tb{Con: High Latency.} 
Along with the accuracy improvement, latency significantly increases.
Even from $2\times$ upscaling, the total $102$ms is much higher than $33$ms of real-time ($30$fps) requirement; the latency of $4\times$ increases up to $126$ms.
We further studies the latency and accuracy tradeoff of high resolution ($1960\times1080$) images. 
Compared to upscaling factors, the original resolution dominates the latency of image enhancement; namely, along with the resolution increasing, though upscaling factor decreases, latency even grows more.
For example, upscaling $980\times540$ image to $1960\times1080$ costs $214$ms. 
%Similar to fixed input resolution, the accuracy also increases along with enhacement because more details have been fed into SR model and inference model.
Current enhancement-based solution works well in video on demand (\eg, \cite{yeo_neural_nodate, yeo_nemo_2020, kim_neural-enhanced_2020}), but to more latency-serious analytics task (not only enhancement but also includes inference latency), prior approaches (\eg, \cite{wang_enabling_nodate, wang_bridging_nodate, yi_eagleeye_2020}) only achieve $2-3$ fps.



\hide{
However, the accuracy of up-scaled image sometimes is not as good as we supposed.
%
For instance, the accuracy of up-scaled frames for 270p and 360p is a little bit lower than low-resolution frame.
%
The reason is for those too blurred video (270p and 360p) containing too less information. 
For small-size object, information is not enough for SR reconstruction; for large-size object, information blurred video pixels generated by SR model with large upscaling factors break the} %the impact most of objects are big enough to be detected in low-resolution frame; up-scaled frames contain fake pixels reconstructed by SR model and hence impact the inference results.
%
%To tackle this problem, we are going to try use region proposal network (RPN) \cite{DBLP:journals/corr/RenHG015} to filter the object which are big enough to be well detected in low-resolution frames.

\hide{
\begin{table}[h]\footnotesize
%\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{-5pt}
\caption{\textbf{Latency and accuracy trade-off}}\label{Tab:Scale&infer}
\begin{center}
\begin{tabular}{c|c|c|c|c}
\hline
\multirow{2}*{\textbf{Resolution}}&\multirow{2}*{\textbf{Scale}}&\multicolumn{2}{c|}{\textbf{Latency (ms/frame)}}&\multirow{2}*{\textbf{Accuracy}}\\
\cline{3-4}
&&\textbf{SR}&\textbf{Infer}\\
\hline
\multirow{2}*{\textbf{270p}} & lr & / & 43.7 &0.845 \\
\cline{2-5}
&$\times 4$&98.0&65.2&0.843\\
\hline
\multirow{2}*{\textbf{360p}} & lr & / & 43.5 &0.890 \\
\cline{2-5}
&$\times 3$&121.3&62.8&0.885\\
\hline
\multirow{2}*{\textbf{540p}} & lr & / & 45.7 &0.911 \\
\cline{2-5}
&$\times 2$&210&86&0.919\\
\hline
\textbf{1080p}&/&/&68&1.00\\
\hline
\end{tabular}
\end{center}
\end{table}
}

%\cb{(optional) GPU usage of existing pipeline is low. Add a preliminary test of these pipelines. VideoStorm is also low usage?}


%%
\subsection{Potential Improvement}\label{subsec:PotentialGain}
%%
Traditional enhancement-participated video analytics based on frame-level, they enhance and infer frame by frame in order of video ingestion.
In this section, we use three real datasets \cite{TrafficCam1, TrafficCam2, TrafficCam3} upscaling them from $640\times360$ to $1280\times720$ to demonstrate the potential improvement of subframe-level enhancement mechanism from spatial. 
From temporal, it brings more potential which we leave to the final experiment.

%%
\subsubsection{Spatial Latency Reduction opportunities.} 
In one single frame, compared to video on demand enhances human quality of experience (QoE) by scaling each frame's resolution \cite{yeo_neural_nodate, yeo_nemo_2020, kim_neural-enhanced_2020}, in video analytics, however, it is crucial that the server-received video has sufficient video quality in the regions that heavily affect the DNN's ability to identify/classify objects; however, the received video does not have to be smooth or have high quality everywhere.
This contrast has a profound implication -- video analytics could achieve high ``quality'' (\ie, accuracy) with much less latency in enhancement. 
Each frame can be spatially enhanced with non-uniform quality levels. 
In object detection, for instance, one may give low quality (\eg, bilinear or bicubic interpolation \cite{Catmull1974ACO}) to the areas other than the objects of interest. 
Fig. \ref{fig:spatiallatencysave} shows that across three datasets (three scenarios), in $60\%-85\%$ frames, the time cost of enhancing only the objects of interest less than $20\%$ of the time cost of enhancing entire frame.

\begin{figure}[h]
\centering
\includegraphics[height=2.1in]{figs/cdf_2.pdf}
\caption{Latency saving opportunities from spatial}
\label{fig:spatiallatencysave}
\end{figure}

%%
\hide{
\subsubsection{Temporal Latency Reduction opportunities.} 
\cb{add a figure like DDS figure 3 but the x-axis is the fraction of enhancement time cost. frame by frame enhance 540P corresponding region of output bbox from 1080P. -> Actually, the enhancement time can be more shorter (we may further reduce the latency via bits stream information, show in the next tb).}



For example, leverages frame encoding types embedded in bits stream to label important frames (\eg, \cite{zhang2016fast, yeo_nemo_2020} enhances only I frames and SR pixels are then transferred to the other frames.).
From encoding perspective, taking inter-frame encoding in H.26x formats as an instance, one frame may encode relying on another similar frame.
Referring to this idea, inference results from similar frames exist dependency relationship as well (\eg, \cite{liu_edge_2019, zhang_mobipose_2020, chen_glimpse_2015} transfer the inference results to the subsequent frames via optical flow or motion vectors).
}




%First, although prior work also reduce latency by tracking pipeline, in decoding step, it treats all the frames equally then feeding them into different pipelines via classifier outside decoder. % for inference \cb{and hence yield} sub-optimal results.
%%
%In contrast, we take all the considerations in compressed space (\ie, in decoder); by doing so, our approach saves the time decoding bit stream into bitmaps (frames).
%%
%Second, DDS and Ekya do not consider the errors made by DNN itself because DDS uses the different compressed-level video but same DNN generateing ground truth while Ekya leverages the same compressed-level video but deeper DNN.
%%
%
%P2: Comparison of the experimental results of previous VAP with/without our decoder.

%%

\hide{
\cb{Online Training on ground truth with SR is better than on generated inference label with inference NN ?} with one figure shows the accuracy gain-latency tradeoff results of online training on Cityscapes: high-cost detect result


%%
%\cb{(Compressed Video Action Recognition, CVPR'18) Why is this better? First, video compression removes up to two orders of magnitude of superfluous information, making interesting signals prominent. Second, the motion vectors in video compression provide us the motion information that lone RGB images do not have. Furthermore, the motion signals already exclude spatial variations, e.g. two people performing the same action in different clothings or in different lighting conditions exhibit the same motion signals. This improves generalization, and the lowered variance further simplifies training. Third, with compressed video, we account for correlation in video frames, i.e. spatial view plus some small changes over time, instead of i.i.d. images. Constraining data in this structure helps us tackling the curse of dimensionality. Last but not least, our method is also much more efficient as we only look at the true signals instead of repeatedly processing near-duplicates. Efficiency is also gained by avoiding to decompress the video, because video is usually stored or transmitted in the compressed version, and access to the motion vectors and residuals are free.}

\tb{Summary.} Third, rich information that may improve VAPs' performance in decoder has not been excavated.
%
Our approach contains two core ideas: 1. leverage image enhanced model to save bandwidth cost and increase inference accuracy; 2. explore the information from decoder and utilize them to speed up image enhancement and DNN inference.
}


%\begin{figure}[t]
%\centering
%\includegraphics[height=1.1in]{figs/VAPDesignSpace.pdf}
%\caption{\normalfont{\emph{Design space of video analytics pipeline.}}}
%\label{fig:IllustrationofVAPworkflow}
%%\vspace{-0.4em}
%\end{figure}



%
%some other VAPs dynamic adjusting camera configuration   corresponds to various network condition. temporal redundancy, spatial redundancy.
%
%From spatial dimension, DDS  filters   while EDDR \cite{} and GRACE \cite{} allocate different quantization parameter to different area.

%%

%%
%Recent advances in video analytics  \cite{lee_mobisr_2019, yi_eagleeye_2020, wang_bridging_nodate, wang_enabling_nodate, yi_supremo_2020} explore a new design space for accuracy enhancing using client-side computation independent of the network bandwidth. 
%
%In particular, they apply neural super-resolution on video frames to enhance detailed information.

%It can also be serve as a streaming protocol/video analytics pipeline. 



%%
%(Good sentence) \cb{In its core,} GRACE is a novel algorithm that designs the compression strategy P for the compression target D. \cb{In what follows,} we first introduce how to estimate the perception model of D in \S4.3 and \S4.4, then we elaborate the optimization algorithms that customize the compression strategies per the estimated perception model in \S5.1 and \S5.2.


\hide{
\textbf{Design space.} 
%
Commonly, the fundamental aim in video analytics is the tradeoff between inference accuracy and bandwidth cost. 
%
Accordingly, we discuss the video analytics pipe-lines along these two dimension:
}
%
%%
\tb{What is new about AccDecoder? (Contributions)}  
%
Prior work (\eg, \cite{chen_glimpse_2015, li_reducto_2020, xu_approxdet_2020, kang_noscope_2017, hsieh_focus_18, liu_edge_2019}) reduces latency by hybrid using light-weight method (often consists of a \emph{detector} and a \emph{tracker}) and the heavy-weight method (a full DNN, \eg, \cite{conf/nips/RenHGS15}).
The light-weight method is like a shortcut to fast process unimportant data and reserve more time windows for heavy-weight but accurate inference.
\emph{Detector}, a fast classifier (\eg, using learned features \cite{kang_noscope_2017, hsieh_focus_18, kang_noscope_2017} or hand-craft low-level image features \cite{chen_glimpse_2015, li_reducto_2020, xu_approxdet_2020}), classifies if the current frame is worth feeding into full DNN for inference; if not, reusing the inference results from the previous nearest frame, but leverage \emph{tracker} (\eg, object tracker \cite{MedianFlow} moves the reused bounding box close to the ground truth) to make up for the accuracy loss from this shortcut.
However, they always assume that bits stream are decoded into frames and the mechanism works on frame-space (see the prior VAPs in Fig. \ref{fig:VAPsCompare}).
These VAPs are from the perspective of the final DNNs, \ie, the export of VAPs, whose inference is frame by frame.
In contrast, we seek to take into account the mechanism works in compressed-video-space (see our decoder in Fig. \ref{fig:VAPsCompare}); namely, we design VAP from the perspective of bits stream (the import of VAPs).
So our approach can be viewed as complementary to this body of prior work.


%%
\hide{
\cite{Hanyao2021edge} Moreover, the deviation of online on-device tracking regarding the objects can only be revealed after the actual inference, which hampers us from efficient online decisions. -> Our method works on compressed video domain. The deviation of tacking of existing work can only revealed after the image rendering, which hampers us from fast decision.
Hybrid using light-weight method (often consists of a \emph{detector} and a \emph{tracker}) and heavy-weight method (a full DNN, \eg, \cite{conf/nips/RenHGS15}) is a typical way to speedup inference.
The light-weight method is like a shortcut to fast process unimportant data and reserve more time window for heavy-weight but accurate inference.
\emph{Detector}, a fast classifier (\eg, using learned features \cite{kang_noscope_2017, hsieh_focus_18} or hand-craft low-level image features \cite{chen_glimpse_2015, li_reducto_2020, xu_approxdet_2020}), classifies if current frame is worth to feed into full DNN for inference; if not, reusing the inference results from the previous nearest frame, but leverage \emph{tracker} (\eg, object tracker \cite{MedianFlow} moves the reused bounding box close to the ground truth) to make up for the accuracy loss from this shortcut.
We note that the video feed mitigation method for saving bandwidth can also reduce computation cost (\eg, \cite{jiang_chameleon_2018, zhang_live_nodate}) and inference latency.
}


%%
% \begin{figure}[h]
% \centering
% \includegraphics[height=2in]{chapters/AccDecoder/figs/VAPsCompare.pdf}
% \caption{Comparison between our design and prior VAPs}
% \label{fig:VAPsCompare}
% \end{figure}


\begin{table*}[t]\footnotesize
\caption{\sout{Comparison between AR/VR/MR and Video Analytics}\wnote{We do not claim bitstream any more in this paper.}}\label{Tab:ARandVA}
\begin{tabular}{m{2cm}|m{3.5cm}|m{3.5cm}|m{3.5cm}}
\hline
\textbf{Application}&\textbf{Latency Constraints}&\textbf{Network Condition}&\textbf{Streaming Unit}\\
\hline
\hline
\textbf{AR/VR/MR \cite{liu_edge_2019, yi_eagleeye_2020, yi_supremo_2020, xu_approxdet_2020, zhang_mobipose_2020, chen_glimpse_2015, zhang_elf_2021}}&\textbf{$\geq60$fps (render one frame within $16.66$ ms)}. Because of the interaction between the user and their wearable device, latency constraints in AR/VR/MR is serious.&\textbf{Ideal network condition.} Desktop/Game Consoles placed in the same space with wearable devices. RTT commonly costs \textbf{$3$ms} \cite{liu_edge_2019}&\textbf{Picture delivery.} Due to the latency constraint, AR/VR/MR can not wait to record and encode multiple frames then delivered. But the ideal network has ability to support picture delivery encoded by JPEG or PNG.\\
\hline
\textbf{VAP \cite{zhang_awstream_2018, du_server-driven_2020, du_AccMPEG_2022, jiang_chameleon_2018, li_reducto_2020, wang_enabling_nodate, wang_bridging_nodate}}&\textbf{$25$fps-$30$fps}. Commonly, the video analytics system processes real-time video.&\textbf{Dynamic and unstable network condition.} Video delivery often cross Wide Area Network (WAN) which cost \textbf{$20-50$ms} RTT and the \textbf{bandwidth is not stable} \cite{awstream}. &\textbf{Video streaming.} Due to the delivery over WAN, streaming by frames too large to be feasible. Moreover, the latency constraint is not that serious.\\
\hline
\end{tabular}	
\end{table*}

%%
The advantages of the design from the perspective of bits stream summarized as follows.
\begin{enumerate}
	\item \emph{Overcome the unstable network condition.} Frame-by-frame processing works well in AR/MR/VR applications, but this only suits ideal network condition whose delivery latency (\~3ms) and bandwidth (one-hop WiFi) is very well (see Table \ref{Tab:ARandVA}); VAPs crossing Wide Area Network (WAN), bits stream delivery tackles the challenge from dynamic bandwidth and network contention. 
	\item \emph{Eliminate unnecessary decoding time costs.} VAPs deliver bits stream with TCP or UDP over WAN. Compressed-video-space mechanism avoids the time waste on decoding bits stream into unnecessary frames/regions (\eg, the second frame of two continuous ones containing static content).
	\item \emph{Make the best of the information in hand.}  Bits stream removes up to two orders of magnitude of superfluous information, making interesting signals prominent. In compressed-video-space, we account for correlation in video frames instead of prior mechanisms designed on \emph{i.i.d.} frames. They repeatedly process near-duplicates to find out ``important'' content by eliminating redundant information among frames. Previous VAPs neglect the information from the codec. %frame then comparing them among continuous frames (for important frame) or in one single frame (for important region); however, they neglect information in codec and repeatedly processing near-duplicates. 
		Obviously, there is a gap between codec and DNN model, however, our key intuition is that \emph{the codec information in hand (\eg, encoding types\footnote{In CV community, some approaches \cite{zhang_fast_2017, wu_compressed_2018, ghodrati_frameexit_2021, wang_fast_2019}, leverage frame types (intra-frame (called I frame) and inter-frame (Non-I frame)) to label important frames. (Actually, H.26x formats adopt multiple types, we naively discussed here with 2 types.) I frames keep the most low-level (pixel-level) information in bits stream. Conceptually, I frames provide DNN model the most low-level information for abstract high-level (semantic-level) one.}), while not accurate, is sufficient to reveal ``important'' content, thereby speeding up video analytics}. 
	%Frame-space mechanisms borrow the idea of video encoding designing their frame filtering mechanism and executing on the frames outputted from the decoder, thus introduce extra latency. The root reason is that prior studies separately design every component rather than holistic consider entire VAP system, and thus neglect information in hand. 
\end{enumerate}

%Computer vision community treat CV tasks on video as an algorithm/model design problem, researchers focus on presenting novel and general models; accordingly and naturally, their studies are short of systematic consideration from video analytics applications. Studies in networking community reveals the strengths (\eg, increase accuracy) and weaknesses (\eg, feed amount of data into wide area network) of distributed VAPs. However, all VAPs do not make full use of video codec information; many of them \cite{chen_glimpse_2015, liu_edge_2019, zhang_mobipose_2020} borrow the idea of video encoding designing their frame filtering mechanism and executing on the frames outputted from the decoder, thus introduce extra latency. The root reason is that prior studies separately design every component rather than holistic consider entire VAP system, and thus neglect information in hand. 



\hide{
%%
Video encoding; it first divides the entire frame into macro blocks, then captures both spatial and temporal redundancy among them. 
%
Temporal redundancy, occupying a dominant position in video redundancy, represents similarities between successive frames; to compress it, inter-frame coding encodes the difference between adjacent frames to compresses a motion picture.
%
DNN inference model learns high-level features from a complex low level representation of data; it abstracts semantical meaningful features from images.
%
Obviously, here is a gap between encoding and DNN model, however, our key intuition is that \emph{the encoding information (\eg, reference frame and motion vector), while not accurate, is sufficient to reveal what information can be reused, thereby speed up SR enhancement (see \S \ref{sub:SR}) and DNN inference (see \ref{sub:mv})}.
%%
%\emph{However, we are on the side of enhancing only important partial content in partial frames}.
}

\hide{
Reducing inference latency: 1. NN-based frame-skip methods lack real platform implementation and AR/MR delivery frame by frame <> both of them neglect existing information in decoder. 2. Partition DNN model among edge(s)/server(s) and front-end devices (not our scope)

%%
\cb{This part discuss the design space (DDS), new models (Pano, EE3P)}
%%
%Distributed architecture of video analytics pipeline necessitates video delivery after encoding, thus decoder plays the pioneer role for video stream reaching backend.
%
Topic: Rich information in decoder to improve VAP performance has not been explored.
}


%
%Video streaming is crucial for  distributed video analytics pipeline that gather videos from  to 
%1. Many deployed cameras don't have enough computing resource.
%2. Network resource is unstable and limited in wide area network.
%\end{abstract}






==> weijun/Cross-stream_Scheduler.tex <==
\subsection{Cross-stream Scheduler}\label{sec:CrossStreamScheduler}


% Global allocation among streams. Bitrate, \wnote{resolution}, fps, and chunk size, \sout{is the same for one edge as the close deployment by the same community/ government/company.} follows $S^i = \sum_{t=1}^T S_{t}$ where $S_t$ is the feature value of neighboring frames calculated in temporal selection section; further, normalize $S^i$ with $l_1$-norm to obtain the allocation weight s.t. $\sum_i S^i=1$.

